The Importance of Norm Regularization in Linear Graph Embedding: Theoretical Analysis and Empirical Demonstration

Learning distributed representations for nodes in graphs is a crucial primitive in network analysis with a wide spectrum of applications. Linear graph embedding methods learn such representations by optimizing the likelihood of both positive and negative edges while constraining the dimension of the embedding vectors. We argue that the generalization performance of these methods is not due to the dimensionality constraint as commonly believed, but rather the small norm of embedding vectors. Both theoretical and empirical evidence are provided to support this argument: (a) we prove that the generalization error of these methods can be bounded by limiting the norm of vectors, regardless of the embedding dimension; (b) we show that the generalization performance of linear graph embedding methods is correlated with the norm of embedding vectors, which is small due to the early stopping of SGD and the vanishing gradients. We performed extensive experiments to validate our analysis and showcased the importance of proper norm regularization in practice.

==> exp.tex <==

\section{Experiments}
\label{sect:exp}

In this section, we conduct several experiments to further validate the importance of restricting
vector norm in linear graph embedding methods. We also compare the empirical performance of the proposed 
low-norm graph embedding methods against the state-of-the-art graph embedding methods and
several other baselines on two tasks: link prediction and node label classification.

\subsection{Experimental Settings}

\vpara{Data Sets:} We use the following three datasets in our experiments:

\begin{itemize}
	\item \tweet is an undirected graph that encodes keyword co-occurrence relationships
using Twitter data. To construct this graph, we collected $\sim$1.1 million
English tweets using Twitter's Streaming API during 2014 August. From the
collected tweets, we extracted the most frequent 10,000 keywords as graph nodes
and their co-occurrences as edges. All nodes with more than 2,000
neighbors are then removed as stop words. There are 9,913 nodes and 681,188 edges in total.
\item \blog~\cite{Zafarani+Liu:2009} is an undirected graph that contains the social 
relationships between BlogCatalog users. It consists of 10,312 nodes and 333,983 undirected 
edges, and each node belongs to one of the 39 groups.
\item \yt~\cite{mislove-2007-socialnetworks} is a social network 
among YouTube users.  It includes 500,000 nodes and 3,319,221 undirected edges\footnote{Available 
	at http://socialnetworks.mpi-sws.org/data-imc2007.html. 
	We only used the subgraph induced by the first 500,000 nodes since our machine 
	doesn't have sufficient memory for training the whole graph. The original graph
	is directed, but we treat it as undirected graph as in \cite{Tang2015}.}.
There are also 30,085 groups, with each group containing $\sim9$ users on average.
\end{itemize}

\vpara{Methods:} The following variants of linear embedding methods are evaluated in our experiments:

\benum{ 
	\item \mmsgd uses the SGD algorithm to optimize the standard linear graph embedding
	objective (Eqn~(\ref{eqn:obj_2})) as in \lne~\cite{Tang2015}.
	
	\item \mmv uses the DCD algorithm to optimize the low-norm objective function 
	(Eqn~(\ref{eqn:hinge_obj})).
	
	\item \mmp uses the DCD algorithm to optimize the pairwise low-norm objective
	function (Eqn~(\ref{eqn:pairwise_hinge})).
	
	\item \mmk optimizes the dual form of low-norm objective function over 
	the kernel matrix instead of explicit embeddings. 
}

\noindent Additionally, we also compare against the following baselines:

\benum{ 
	\item \nv \cite{GroverL16} is a state-of-the-art graph embedding method.
	Compared with \lne \cite{Tang2015}, it uses random walks to sample nodes as positive
	neighborhoods for graph nodes, while \lne uses direct neighbors in the
	original graph. 
	
	\item \cn \cite{Liben-NowellK03} is a simple yet strong baseline for link
	prediction. Given two nodes $u$ and $v$, it computes the score between $u$
	and $v$ as $\text{score}(u, v) = |N_+(u) \cap N_+(v)|$, namely the number of
	common neighbors between $u$ and $v$.
	
	\item \svd computes the Singular Value Decomposition of the adjacency matrix to obtain
	low-dimensional representations for graph nodes.
	
	\item \grf~\cite{zhu2003semi} is a semi-supervised learning method 
	for node label classification on graph. It first sets the score of each labeled node as $0$ 
	or $1$, then repeatedly updates the score of unlabeled nodes as the average score
	 of nodes in its neighborhood until convergence. 
}

For \nv\footnote{http://snap.stanford.edu/node2vec/}, we obtained the
implementation from the original paper. For \svd, we used the 
Randomized SVD algorithm~\cite{halko2011finding} in Scikit-learn~\cite{pedregosa2011scikit}.
For all the other methods, we implemented them in C++. All three datasets are
partitioned into three parts for training, validating and testing respectively.
The size ratio of the three parts are 2:1:1 for all datasets. We conducted
all the experiments on a Windows machine with Xeon E3 3.4GHz CPU and 8GB memory. 
Other details about the experimental protocols and parameter settings are omitted
here due to page limitations, and can be found \techreport{in the appendix}\paper{in our technical report~\cite{TechReport}}.

\subsection{Additional Experiments on Importance of Vector Norm Restriction}

In this section, we conduct several experiments to evaluate \mmsgd and low-norm 
methods on datasets \blog and \yt. These experiments complement the ones in
Section~\ref{sect:norm} and~\ref{sect:method} to further validate the importance
of restricting vector norm for linear graph embedding methods.

In the first set of experiments, we further demonstrate the early stopping effect of SGD. 
As in Section~\ref{sect:norm}, we run the SGD algorithm to optimize \mmsgd objective 
and stop the iterations after a certain period of time. Figure~\ref{fig:blog_AP} 
and~\ref{fig:blog_F1} shows the link prediction AP score and the node classification macro 
F1 score on \blog respectively. As we can see, the generalization AP score for link prediction 
peaks at around $10$ epochs, which is similar to what we have observed in Section~\ref{sect:sgd}. 
The early stopping effect on macro-F1 score for node label classification is less apparent, 
probably due to the post-processing SVM step compensating for it. However, we still observed
the performance drop after around $50$ epochs (not shown in the figure).

\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_blog_AP.png}
		\vspace{-15pt}
		\caption{Link Prediction}\label{fig:blog_AP}
	\end{subfigure}%
	~ 
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_blog_F1.png}
		\vspace{-15pt}
		\caption{Node label Classification}\label{fig:blog_F1}
	\end{subfigure}
	
	\vspace{-10pt}
	\caption{Early Stopping Effect on \blog Dataset}\label{fig:blog}
\end{figure}


The next set of experiments compare the efficiency of \mmsgd(SGD) and \mmv(DCD) on \blog 
and \yt datasets. Figure~\ref{fig:efficiency_2} shows the testing AP score over the course 
of training procedure for both datasets. As we can see, the DCD algorithm converges faster 
than the SGD algorithm on both datasets, reaching optimal performance at around $6.4$ seconds 
for \blog dataset and $61$ seconds for \yt dataset. On the other hand, the SGD algorithm has
not yet completely converged even after $11.2$ seconds for \blog dataset and $81$ seconds for 
\yt dataset.

\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_blog_efficiency.png}
		\vspace{-15pt}
		\caption{\blog Dataset}\label{fig:blog_efficiency}
	\end{subfigure}%
	~ 
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_youtube_efficiency.png}
		\vspace{-15pt}
		\caption{\yt Dataset}\label{fig:youtube_efficiency}
	\end{subfigure}
	
	\vspace{-10pt}
	\caption{Efficiency Comparison}\label{fig:efficiency_2}
\end{figure}

In the final set of experiments, we demonstrate the importance of choosing appropriate value for 
the norm regularization parameter $\lambda_r$. Figure~\ref{fig:reg} shows
the testing AP score of \mmv with varying value of $\lambda_r$ on \blog and \yt datasets.
Similar to what we have observed previously in Section~\ref{sect:method}, the regularization 
parameter $\lambda_r$ controls the model capacity, which affects the generalization
performance. Therefore, finding the optimal value of $\lambda_r$ is the key for achieving good
generalization performance for low-norm embedding methods.

\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_blog_reg.png}
		\vspace{-15pt}
		\caption{\blog Dataset}\label{fig:blog_reg}
	\end{subfigure}%
	~ 
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width = 3.5cm]{figure/fig_youtube_reg.png}
		\vspace{-15pt}
		\caption{\yt Dataset}\label{fig:youtube_reg}
	\end{subfigure}
	
	\vspace{-10pt}
	\caption{Efficiency Comparison}\label{fig:reg}
\end{figure}


\subsection{Link Prediction Performance}\label{sect:link_prediction}

Table~\ref{tbl:link_prediction} shows the performance of all methods on the link prediction 
task\footnote{We are unable to report the performance of \nv, \grf and \mmk on \yt, since 
they do not scale well to this large dataset.}.
As we can see, the linear graph embedding methods consistently outperform all baselines. 
Among the four linear graph embedding methods, \mmp provides slightly better
performance across all datasets. \mmsgd slightly outperforms \mmv on \tweet and \blog datasets, but such performance requires both the optimal parameter configuration and sufficiently
long training time to achieve. As a result, \mmsgd would be considerably worse compared to \mmv 
and \mmp for larger datasets (such as \yt), due to the fact that parameter tuning and actual training are very costly in such scenario. 



% graph that encodes the Protein-Protein
% Interactions for Homo Sapiens. There are 3,890 nodes and 76,584 undirected
% edges in this graph.

\subsection{Node Label Classification Performance}

Table~\ref{tbl:node_classification} shows the performance on the node label classification task. On 
\blog dataset, \nv achieved the best performance overall, which confirms earlier findings in \cite{GroverL16} that adding additional positive neighbors generated from random walk would improve 
the label classification accuracy. We remark that the technique used in \nv~\cite{GroverL16} is 
also applicable to our low-norm formulation, and hence it is promising that such a technique can 
also lead to performance improvement. Overall, the linear graph embedding methods significantly
outperform all other baselines, achieving $\sim 2$ and $\sim 10$ times better F1-score on \blog 
and \yt respectively. Among the four linear graph embedding variants, \mmp performs slightly 
better across all datasets.

\begin{table}[t]
	\small
	\caption{Link Prediction Performance (AP)}
	\label{tbl:link_prediction}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		& \texttt{CommonNb} & \mmsgd & \nv & \svd & \mmp \\
		\hline
		\tweet & 0.754 & 0.753 & 0.390 & 0.737 & 0.754 \\
		\blog & 0.794 & 0.865 & 0.545 & 0.854 & \textbf{0.871} \\
		\yt & 0.755 & 0.883 & N/A & 0.811 & \textbf{0.903} \\
		\hline 
		& \multicolumn{4}{|c|}{\mmv} &  \\
		\cline{2-5}
		& $\lambda_r = 1$ & $\lambda_r = 3$ & $\lambda_r = 5$ & $\lambda_r = 10$ & \mmk \\		
		\hline
		\tweet & 0.677 & 0.741 & 0.750 & 0.728 & \textbf{0.755} \\
		\blog & 0.819 & 0.857 & 0.840 & 0.839 & 0.863 \\
		\yt & 0.871 & 0.896 & 0.879 & 0.854 & N/A  \\
		\hline
	\end{tabular}
\end{table}

\begin{table}[t]
	\small
	\caption{Node Label Classification Performance (Macro-F1)}
	\label{tbl:node_classification}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		& \grf & \mmsgd & \nv & \svd & \mmp \\
		\hline
		\blog & 0.074 & 0.143 & \textbf{0.172} & 0.044 & 0.149 \\
		\yt & N/A & 0.0035\footnote{Based on our experimental results on other datasets, the performance of \mmsgd is comparable with low-norm methods when using the optimal configuration and with sufficiently long training time. However due to the large scale of \yt dataset, we were unable to search extensively for the optimal configuration of \mmsgd, thus resulting in the relatively worse reported performance on both tasks.} & N/A & 0.0027 & \textbf{0.0359} \\
		\hline
		& \multicolumn{4}{|c|}{\mmv} &  \\
		\cline{2-5}
		& $\lambda_r = 1$ & $\lambda_r = 3$ & $\lambda_r = 5$ & $\lambda_r = 10$ & \\		
		\hline
		\blog & 0.131 & 0.137 & 0.135 & 0.064 &  \\
		\yt & 0.0318 & 0.0331 & 0.0198  & 0.0042 &   \\
		\hline
	\end{tabular}
\end{table}

\subsubsection{Efficiency Comparison} Figure~\ref{fig:efficiency} demonstrates the empirical comparison
of training efficiency between SGD and DCD algorithms (both with optimal parameter configuration). For 
fair comparison, the $x$-axis is the total running time (in seconds) and $y$-axis shows the link 
prediction AP score on testing dataset. As we can see, the DCD algorithm converges much faster than 
the SGD algorithm: it takes only about $15$ seconds to converge while the SGD algorithm still has not converged even after $30$ seconds. Note that after about $100$ epochs (not shown in the figure), the SGD algorithm could achieve similar performance as the DCD algorithm, but it requires significantly longer training time (Figure~\ref{fig:efficiency} only shows the trend up to $20$ epochs).

\begin{figure}[h]
	\centering
	\includegraphics[width=5cm]{figure/fig_efficiency.png}
	\vspace{-10pt}	
	\caption{Efficiency Comparison}
	\label{fig:efficiency}
	\vspace{-10pt}	
\end{figure}

==> iclr/Master-Template-ICLR2019/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related.tex <==
\section{Other Related Work}
\label{sect:related}

Classical graph embedding algorithms such as multidimensional scaling (MDS)
\cite{kruskal1978multidimensional}, IsoMap \cite{tenenbaum2000global}, and
Laplacian Eigenmap \cite{belkin2001laplacian} typically construct an affinity
graph with the features of the given data points, and then look for
low-dimensional representations of the data points based on the graph. These
methods typically require finding the eigenvectors of the affinity matrix,
making them hard to scale on large graphs with millions of nodes.

% mainly perform dimension reduction for the
% features of graph nodes.  They try to generate low-dimensional manifolds that
% capture non-linear geometry of the data. Such methods include  They are not scalable enough. 

In recent years, the success of Word2Vec \cite{mikolov2013distributed} has
inspired a handful of neural-network-based techniques for graph embedding:
\begin{itemize}[leftmargin=1.5em]
	\item Perozzi \etal \cite{Perozzi2014} propose the DeepWalk method,
	that first uses random walks to generate a large number of paths from the
	graph, and then applies the SkipGram model to learn vectorized representations
	for graph nodes.
	\item Tang \etal \cite{Tang2015} use node embeddings to model the
	neighborhood distributions of graph nodes, and learn the embeddings such that
	the embedding-based distributions align well with the empirical distributions.
	\item Grover \etal \cite{GroverL16} propose the Node2Vec method, which uses a biased
	random walk procedure to obtain expanded neighborhoods for graph nodes instead
	of the observed neighbors.
\end{itemize}
All of these methods fall within the generic framework of linear graph embedding, 
with differences primarily on the construction of proximity matrix, so our analysis 
applies to all these methods.

% However, as aforementioned, 
% the generalization performance of these methods are likely due to the regularization
% effect of early stopping, which makes these methods sensitive to parameter choices.
% As we shall see in this paper, by adding strong explicit regularization terms, the 
% low-norm embedding methods could achieve significantly better 
% performance.
	
% the inner products of node embeddings to preserve the graph structure, they
% cannot capture the non-linear interactions between node embeddings to preserve
% graph structures more accurately.


Apart from the linear graph embedding techniques listed above, there are also
studies \cite{li2014lrbm, TianGCCL14, LiTBZ15, wang2016structural}
that use deep neural network architectures to preserve graph
structures.  However, these methods usually require a large training time
and are sensitive to neural network hyper-parameters.  Moreover, it is very 
difficult to theoretically analyze these methods. Hence, it remains
unclear what level of generalization accuracy these methods can achieve.

Learning embedding vectors with norm constraints and hinge-loss has been proposed
by Srebro \etal \cite{srebro2005maximum} as an alternative to low-rank factorization
(i.e., SVD). However, Srebro \etal put constraint on the trace norm of the
reconstructed proximity matrix, and the resulting objective function requires a generic 
semi-definite programming (SDP) solver, which has severe scalability issues. 

Dual Coordinate Descent (DCD)~\cite{HsiehCLKS08} is an optimization algorithm 
originally designed for solving SVM. Due to the connection between SVM and our
low-norm embedding objective , it can also be adapted as a building block for 
learning low-norm graph embedding (details will be discussed in this paper). 


==> theory.tex <==
\vspace{-10pt}
\section{Generalization Analysis of Linear Graph Embedding Methods}
\label{sect:theory}

The first major point of this paper is to argue that the generalization of linear graph embedding
methods in Section~\ref{sect:prelim} are more likely determined by the norm of embedding vectors
instead of their dimensions. 
We begin by providing a theoretical generalization error analysis
of linear graph embedding that characterizes the importance of restricting the
norm of vectors. We consider the following statistical model for graph generation: 
assume that there exists an unknown probability distribution $\mathcal{Q}$ over the
Cartesian product $V \times U$ of two vertex sets $V$ and $U$. Each sample $(a,b)$ 
from $\mathcal{Q}$ denotes an edge connecting $a \in V$ and $b \in U$.The graph that
we observed consists of the first $m$ i.i.d. samples from the distribution $\mathcal{P}$, 
and the goal is use these $m$ samples to learn a model that generalizes well to the 
underlying distribution $\mathcal{P}$. Note that in the above notations, we allow 
either $V = U$ for homogeneous graphs or $V \cap U = \emptyset$ for bipartite graphs. 

Define  $\mathcal{U}$ to be the uniform distribution over $V \times U$ for generating 
the negative edges, and $\mathcal{P}$ be the combined distribution over $V \times U 
\times \{\pm 1\}$ that generates both positive and negative edges (i.e., $(a,b,+1)$ 
indicates that $(a,b)$ is sampled from $\mathcal{Q}$, and $(a,b,-1)$ indicates otherwise). 
Intuitively, a good graph embedding should be able to distinguish whether a future sample 
from $\mathcal{P}$ is actually sampled from $\mathcal{Q}$ or $\mathcal{U}$. Using the above 
notations, we have the following theorem which bounds the generalization error of a linear 
embedding model on the link prediction task:

\begin{theorem}\label{thm:bipartite}% [Generalization Error of Max-Margin Graph Embedding]
	Let $E = \{(a_1, b_1, y_1), (a_2, b_2, y_2), \ldots, (a_{m+m'}, b_{m+m'}, y_{m+m'})\}$ 
	be i.i.d. samples from a distribution $\mathcal{P}$ over $V \times U \times \{\pm 1\}$. 
	Let $\x_1, \x_2, \ldots, \x_n$ be the embedding vectors for nodes $v_1, v_2, \ldots, v_n$ 
	$V$ and $\t_1, \t_2, \ldots, \t_k$ be the embedding vectors for nodes $u_1, \ldots, u_k$ 
	in $U$. Then for any $1$-Lipschitz loss function $\mathcal{L} : \mathbb{R} \rightarrow 
	[0, C]$ and $C_x, C_t$, with probability $1 - \delta$:
	\begin{align*}
		& \forall \x,\t, \quad \textit{s.t.} \quad \sum_{i=1}^n \norm{\x_i}^2 \leq C_x, \sum_{j=1}^k \norm{\t_j}^2 \leq C_t, \\
	& \mathbb{E}_{(a,b,y) \sim \mathcal{P}} \mathcal{L}(y \x_a^T \t_b) \leq \frac{1}{m+m'} \sum_{i=1}^{m+m'} 
	\mathcal{L}(y_i \x_{a_i}^T \t_{b_i}) + \frac{2}{m+m'} \mathbb{E}_\sigma ||A_\sigma||_2 \sqrt{C_x C_t} + 4 C \sqrt{\frac{2 \ln (4 / \delta)}{m+m'}}
	\end{align*}
	where $||A_\sigma||_2$ is the spectral norm of the random matrix $A_\sigma$ defined as follows:
	\begin{align*}
	A_\sigma(i,j) = \left\{
	\begin{array}{lr}
	\sigma_{ij} & \exists y, (i, j, y) \in E \\
	0 & \forall y, (i,j,y) \notin E \\
	\end{array}
	\right.
	\end{align*}
	in which $\sigma_{ij}$ are i.i.d. Rademacher random variables.
\end{theorem}

The proof of this theorem can be found in the appendix. As we can see, our generalization error analysis 
does not depend on the embedding dimension. Therefore, we can enjoy good generalization performance by 
ensuring the total squared norm of embedding vectors is small, even if the embedding dimension is very large.

For homogeneous graphs, we have the following corollary, which is obtained by restricting $U = V$ and $\t_i = \x_i$ in Theorem~\ref{thm:bipartite}:

\begin{corollary}\label{thm:graph}% [Generalization Error of Max-Margin Graph Embedding]
	Let $E = \{(a_1, b_1, y_1), (a_2, b_2, y_2), \ldots, (\{a_{m+m'}, b_{m+m'}\}, y_{m+m'})\}$ be i.i.d. 
	samples from a distribution $\mathcal{P}$ over $V \times V \times \{\pm 1\}$. Let $\x_1, \x_2, \ldots, 
	\x_n$ be the embedding vectors for nodes $v_1, \ldots, v_n$, then for any $1$-Lipschitz loss function 
	$\mathcal{L} : \mathbb{R} \rightarrow [0, C]$ and $C_x$, with probability $1 - \delta$:
	\begin{align*}
	& \forall \x, \quad \textit{s.t.} \quad \sum_{i=1}^n \norm{\x_i}^2 \leq C_x, \\
	& \mathbb{E}_{(a,b,y) \sim \mathcal{P}} \mathcal{L}(y \x_a^T \x_b) \leq \frac{1}{m + m'} \sum_{i=1}^{m+m'} 
	\mathcal{L}(y_i \x_{a_i}^T \x_{b_i}) + \frac{2}{m+m'} \mathbb{E}_\sigma ||A_\sigma||_2 C_x + 4 C \sqrt{\frac{2 \ln (2 / \delta)}{m + m'}}
	\end{align*}
\end{corollary}


We suspect that the vector norm is also the key factor to the generalization of existing graph
embedding methods: although not explicitly regularized, the norm of embedding vectors are still 
small due to the relatively few iterations of SGD executed on each vector\footnote{Most graph 
embedding experiments are conducted on large scale graphs. Therefore, even though the total number 
of iterations are set to be large, the number of iterations executed on each embedding vector is
small.}. The empirical evidences for this argument can be found in Section~\ref{sect:exp}: if we keep
running the SGD procedure in \lne~\cite{Tang2015}, the norm of embedding vectors will continue to
increase, and the generalization performance will start to drop.



